Ethnic Groups' Access to State Power and Group Size

Ethnic-based political inequality is widespread, yet its underlying drivers remain poorly understood. This paper shows that an ethnic group's relative size is a key correlate of its access to central executive power. Using data on 575 groups across 181 countries from 1946 to 2021, I document a robust inverted-U-shaped relationship: groups of intermediate size are significantly more likely to gain political inclusion than both very small and very large ones. A simple model explains this pattern as the result of elite trade-offs between the risks of conflict from exclusion and the costs of sharing political rents. The model further predicts-and the data confirm-that the inverted-U is most pronounced in countries with historically competitive institutions. These findings offer new insight into the joint role of ethnic composition and institutions in shaping patterns of ethnic political inclusion.

==> table5a.tex <==
Relative size       &       2.674\sym{***}&       4.236\sym{***}&       2.563\sym{***}&       4.473\sym{**} &       1.021\sym{**} \\
                    &     (0.513)         &     (1.270)         &     (0.858)         &     (2.034)         &     (0.436)         \\
Relative size squared&      -3.824\sym{***}&      -8.853\sym{***}&      -2.751\sym{**} &      -5.770\sym{**} &                     \\
                    &     (0.831)         &     (3.150)         &     (1.287)         &     (2.622)         &                     \\
Joint significance  &       0.000         &       0.003         &       0.014         &       0.095         &                     \\
Vertex              &       0.350         &       0.239         &       0.466         &       0.388         &                     \\
R-squared           &       0.609         &       0.891         &       0.593         &       0.875         &       0.581         \\
Observations        &        1813         &        1798         &        1156         &        1150         &        1156         \\


==> table6.tex <==
Relative size       &       3.703\sym{***}&       2.103\sym{***}&       0.852\sym{**} &       3.954\sym{***}&       3.954\sym{***}&       1.373\sym{***}\\
                    &     (0.577)         &     (0.787)         &     (0.401)         &     (0.603)         &     (0.603)         &     (0.386)         \\
Relative size squared&      -4.912\sym{***}&  -2.460\sym{\dagger}&                     &      -5.263\sym{***}&      -5.263\sym{***}&                     \\
                    &     (0.843)         &     (1.511)         &                     &     (0.883)         &     (0.883)         &                     \\
Joint significance  &       0.000         &       0.016         &                     &       0.000         &       0.000         &                     \\
Vertex              &       0.377         &       0.428         &                     &       0.376         &       0.376         &                     \\
R-squared           &       0.582         &       0.646         &       0.640         &       0.608         &       0.608         &       0.581         \\
Observations        &        4668         &        2597         &        2597         &        5136         &        5136         &        5136         \\


==> tableIIIa.tex <==
Relative size       &       1.650\sym{***}&       1.646\sym{***}&       1.645\sym{***}&       1.658\sym{***}&       1.658\sym{***}\\
                    &     (0.330)         &     (0.329)         &     (0.328)         &     (0.326)         &     (0.327)         \\
Relative size squared&      -1.762\sym{***}&      -1.759\sym{***}&      -1.758\sym{***}&      -1.770\sym{***}&      -1.770\sym{***}\\
                    &     (0.347)         &     (0.346)         &     (0.346)         &     (0.344)         &     (0.344)         \\
Joint significance  &       0.000         &       0.000         &       0.000         &       0.000         &       0.000         \\
Vertex              &       0.468         &       0.468         &       0.468         &       0.468         &       0.468         \\
R-squared           &       0.052         &       0.055         &       0.059         &       0.065         &       0.066         \\
Observations        &      821832         &      821832         &      821832         &      821832         &      821832         \\


==> tableIIIb.tex <==
Relative size       &       1.642\sym{***}&       1.638\sym{***}&       1.637\sym{***}&       1.650\sym{***}&       1.649\sym{***}\\
                    &     (0.342)         &     (0.341)         &     (0.341)         &     (0.339)         &     (0.339)         \\
Relative size squared&      -1.746\sym{***}&      -1.742\sym{***}&      -1.741\sym{***}&      -1.754\sym{***}&      -1.753\sym{***}\\
                    &     (0.360)         &     (0.358)         &     (0.358)         &     (0.356)         &     (0.356)         \\
Joint significance  &       0.000         &       0.000         &       0.000         &       0.000         &       0.000         \\
Vertex              &       0.470         &       0.470         &       0.470         &       0.470         &       0.470         \\
R-squared           &       0.054         &       0.058         &       0.060         &       0.067         &       0.068         \\
Observations        &     1568532         &     1568532         &     1568532         &     1568532         &     1568532         \\


==> tableIIIc.tex <==
Relative size       &       3.083\sym{***}&       3.078\sym{***}&       3.077\sym{***}&       3.086\sym{***}&       3.086\sym{***}\\
                    &     (0.278)         &     (0.277)         &     (0.277)         &     (0.276)         &     (0.276)         \\
Relative size squared&      -3.197\sym{***}&      -3.191\sym{***}&      -3.190\sym{***}&      -3.199\sym{***}&      -3.199\sym{***}\\
                    &     (0.290)         &     (0.289)         &     (0.289)         &     (0.288)         &     (0.288)         \\
Joint significance  &       0.000         &       0.000         &       0.000         &       0.000         &       0.000         \\
Vertex              &       0.482         &       0.482         &       0.482         &       0.482         &       0.482         \\
R-squared           &       0.305         &       0.308         &       0.310         &       0.312         &       0.313         \\
Observations        &      836462         &      836462         &      836462         &      836462         &      836462         \\


==> tableIVa.tex <==
Relative size       &       1.700\sym{***}&       1.711\sym{***}&       1.710\sym{***}&       1.706\sym{***}&       1.717\sym{***}\\
                    &     (0.339)         &     (0.337)         &     (0.337)         &     (0.340)         &     (0.338)         \\
Relative size squared&      -1.802\sym{***}&      -1.813\sym{***}&      -1.812\sym{***}&      -1.809\sym{***}&      -1.819\sym{***}\\
                    &     (0.355)         &     (0.353)         &     (0.353)         &     (0.355)         &     (0.353)         \\
Joint significance  &       0.000         &       0.000         &       0.000         &       0.000         &       0.000         \\
Vertex              &       0.472         &       0.472         &       0.472         &       0.472         &       0.472         \\
R-squared           &       0.066         &       0.072         &       0.073         &       0.067         &       0.073         \\
Observations        &      835698         &      835698         &      835698         &      835698         &      835698         \\


==> tableIVb.tex <==
Relative size       &       1.679\sym{***}&       1.684\sym{***}&       1.683\sym{***}&       1.706\sym{***}&       1.717\sym{***}\\
                    &     (0.333)         &     (0.331)         &     (0.332)         &     (0.338)         &     (0.337)         \\
Relative size squared&      -1.784\sym{***}&      -1.789\sym{***}&      -1.789\sym{***}&      -1.808\sym{***}&      -1.820\sym{***}\\
                    &     (0.350)         &     (0.348)         &     (0.348)         &     (0.354)         &     (0.353)         \\
Countries with group&      -0.001\sym{***}&       0.000         &      -0.000         &      -0.001\sym{***}&      -0.000         \\
                    &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
Joint significance  &       0.000         &       0.000         &       0.000         &       0.000         &       0.000         \\
Vertex              &       0.470         &       0.470         &       0.470         &       0.472         &       0.472         \\
R-squared           &       0.066         &       0.073         &       0.073         &       0.069         &       0.075         \\
Observations        &      715390         &      715390         &      715390         &      621845         &      621845         \\


==> tableVIa.tex <==
Relative size       &       3.461\sym{***}&       0.642\sym{*}  &       0.098         &       3.472\sym{***}&       0.624\sym{*}  &       0.096         \\
                    &     (0.557)         &     (0.374)         &     (0.072)         &     (0.569)         &     (0.376)         &     (0.072)         \\
Relative size squared&      -3.636\sym{***}&      -0.685\sym{*}  &                     &      -3.650\sym{***}&      -0.666\sym{*}  &                     \\
                    &     (0.586)         &     (0.392)         &                     &     (0.598)         &     (0.393)         &                     \\
Joint significance  &       0.000         &       0.208         &                     &       0.000         &       0.224         &                     \\
Vertex              &       0.476         &       0.469         &                     &       0.476         &       0.469         &                     \\
R-squared           &       0.216         &       0.027         &       0.019         &       0.209         &       0.015         &       0.008         \\
Observations        &      294949         &      350220         &      350220         &      294949         &      350220         &      350220         \\


==> tableVIb.tex <==
Relative size       &       2.334\sym{***}&       1.172\sym{***}&       0.250\sym{**} &       2.333\sym{***}&       1.165\sym{***}&       0.245\sym{**} \\
                    &     (0.511)         &     (0.439)         &     (0.105)         &     (0.517)         &     (0.442)         &     (0.105)         \\
Relative size squared&      -2.448\sym{***}&      -1.229\sym{**} &                     &      -2.448\sym{***}&      -1.226\sym{***}&                     \\
                    &     (0.524)         &     (0.469)         &                     &     (0.530)         &     (0.473)         &                     \\
Joint significance  &       0.000         &       0.029         &                     &       0.000         &       0.029         &                     \\
Vertex              &       0.477         &       0.477         &                     &       0.477         &       0.475         &                     \\
R-squared           &       0.115         &       0.046         &       0.025         &       0.108         &       0.038         &       0.016         \\
Observations        &      512876         &      322822         &      322822         &      512876         &      322822         &      322822         \\


==> tableVa.tex <==
Relative size       &       3.221\sym{***}&       3.226\sym{***}&   0.570\sym{\dagger}&   0.572\sym{\dagger}&       0.094         \\
                    &     (0.519)         &     (0.519)         &     (0.373)         &     (0.373)         &     (0.070)         \\
Relative size squared&      -3.413\sym{***}&      -3.415\sym{***}&  -0.600\sym{\dagger}&  -0.602\sym{\dagger}&                     \\
                    &     (0.548)         &     (0.548)         &     (0.391)         &     (0.390)         &                     \\
Joint significance  &       0.000         &       0.000         &       0.311         &       0.307         &                     \\
Vertex              &       0.472         &       0.472         &       0.475         &       0.475         &                     \\
R-squared           &       0.196         &       0.199         &       0.026         &       0.030         &       0.024         \\
Observations        &      295378         &      295378         &      350509         &      350509         &      350509         \\


==> tableVb.tex <==
Relative size       &       2.334\sym{***}&       2.334\sym{***}&       1.102\sym{**} &       1.104\sym{**} &       0.236\sym{**} \\
                    &     (0.501)         &     (0.502)         &     (0.432)         &     (0.432)         &     (0.098)         \\
Relative size squared&      -2.458\sym{***}&      -2.458\sym{***}&      -1.150\sym{**} &      -1.151\sym{**} &                     \\
                    &     (0.514)         &     (0.515)         &     (0.463)         &     (0.462)         &                     \\
Joint significance  &       0.000         &       0.000         &       0.032         &       0.031         &                     \\
Vertex              &       0.475         &       0.475         &       0.479         &       0.480         &                     \\
R-squared           &       0.114         &       0.116         &       0.045         &       0.048         &       0.029         \\
Observations        &      513227         &      513227         &      323235         &      323235         &      323235         \\

